Bias and Diversity in Synthetic-based Face Recognition

Synthetic data is emerging as a substitute for authentic data to solve ethical and legal challenges in handling authentic face data. The current models can create real-looking face images of people who do not exist. However, it is a known and sensitive problem that face recognition systems are susceptible to bias, i.e. performance differences between different demographic and non-demographics attributes, which can lead to unfair decisions. In this work, we investigate how the diversity of synthetic face recognition datasets compares to authentic datasets, and how the distribution of the training data of the generative models affects the distribution of the synthetic data. To do this, we looked at the distribution of gender, ethnicity, age, and head position. Furthermore, we investigated the concrete bias of three recent synthetic-based face recognition models on the studied attributes in comparison to a baseline model trained on authentic data. Our results show that the generator generate a similar distribution as the used training data in terms of the different attributes. With regard to bias, it can be seen that the synthetic-based models share a similar bias behavior with the authentic-based models. However, with the uncovered lower intra-identity attribute consistency seems to be beneficial in reducing bias.

==> old_tbles.tex <==
\begin{table*}[]
\centering
\begin{tabular}{c|cccc|rr} \hline \hline
Model & Black & Asian & White & Indian & mAcc + STD   & SER \\ \hline
SFace$_{auth}$                & 92.20   & 87.43 & 95.56     & 90.71  & 91.48$\pm$2.92 & 2.83    \\ \hline
SFace$_{syth}$               & 90.05   & 85.66 & 94.04     & 88.99  & 89.69$\pm$2.99 & 2.41    \\
SynFace                   & 74.92   & 72.79 & 79.47     & 75.90  & 75.77$\pm$2.41 & 1.32    \\
USynthFace                & 75.66   & 74.01 & 80.35     & 77.06  & 76.77$\pm$2.33 & 1.32    \\ \hline \hline
\end{tabular}
\caption{BFW}
\end{table*}

\begin{table*}[]
\centering
\begin{tabular}{c|cccc|rr} \hline \hline
Model & African & Asian & Caucasian & Indian & mAcc + STD    & SER \\ \hline
SFace$_{auth}$            & 85.52   & 84.27 & 92.52     & 88.03  & 87.59$\pm$3.15 & 2.10    \\ \hline 
SFace$_{syth}$            & 80.17   & 80.93 & 90.15     & 84.32  & 83.89$\pm$3.94 & 2.01    \\
SynFace                   & 59.75   & 67.20 & 70.05     & 66.00  & 65.75$\pm$3.76 & 1.34    \\
USynthFace                & 60.25   & 67.67 & 72.40     & 69.13  & 67.36$\pm$4.45 & 1.44    \\ \hline \hline
\end{tabular}
\caption{RFW}
\end{table*}


